MemFusionMap: Working Memory Fusion for Online Vectorized HD Map Construction

High-definition (HD) maps provide environmental information for autonomous driving systems and are essential for safe planning. While existing methods with single-frame input achieve impressive performance for online vectorized HD map construction, they still struggle with complex scenarios and occlusions. We propose MemFusionMap, a novel temporal fusion model with enhanced temporal reasoning capabilities for online HD map construction. Specifically, we contribute a working memory fusion module that improves the model's memory capacity to reason across a history of frames. We also design a novel temporal overlap heatmap to explicitly inform the model about the temporal overlap information and vehicle trajectory in the Bird's Eye View space. By integrating these two designs, MemFusionMap significantly outperforms existing methods while also maintaining a versatile design for scalability. We conduct extensive evaluation on open-source benchmarks and demonstrate a maximum improvement of 5.4% in mAP over state-of-the-art methods. The project page for MemFusionMap is https://song-jingyu.github.io/MemFusionMap

==> egbib_backup.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@InProceedings{yuan2024streammapnet,
    author    = {Yuan, Tianyuan and Liu, Yicheng and Wang, Yue and Wang, Yilun and Zhao, Hang},
    title     = {StreamMapNet: Streaming Mapping Network for Vectorized Online HD Map Construction},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)},
    month     = {January},
    year      = {2024},
    pages     = {7356-7365}
}

@article{chen2024maptracker,
  title={Maptracker: Tracking with strided memory fusion for consistent vector hd mapping},
  author={Chen, Jiacheng and Wu, Yuefan and Tan, Jiaqi and Ma, Hang and Furukawa, Yasutaka},
  journal={arXiv preprint arXiv:2403.15951},
  year={2024}
}

@inproceedings{liu2023vectormapnet,
  title={Vectormapnet: End-to-end vectorized hd map learning},
  author={Liu, Yicheng and Yuan, Tianyuan and Wang, Yue and Wang, Yilun and Zhao, Hang},
  booktitle={International Conference on Machine Learning},
  pages={22352--22369},
  year={2023},
  organization={PMLR}
}

@inproceedings{gu2024producing,
  title={Producing and leveraging online map uncertainty in trajectory prediction},
  author={Gu, Xunjiang and Song, Guanyu and Gilitschenski, Igor and Pavone, Marco and Ivanovic, Boris},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14521--14530},
  year={2024}
}

@inproceedings{
liao2023maptr,
title={Map{TR}: Structured Modeling and Learning for Online Vectorized {HD} Map Construction},
author={Bencheng Liao and Shaoyu Chen and Xinggang Wang and Tianheng Cheng and Qian Zhang and Wenyu Liu and Chang Huang},
booktitle={The Eleventh International Conference on Learning Representations },
year={2023},
url={https://openreview.net/forum?id=k7p_YAO7yE}
}

@article{liao2023maptrv2,
  title={Maptrv2: An end-to-end framework for online vectorized hd map construction},
  author={Liao, Bencheng and Chen, Shaoyu and Zhang, Yunchi and Jiang, Bo and Zhang, Qian and Liu, Wenyu and Huang, Chang and Wang, Xinggang},
  journal={arXiv preprint arXiv:2308.05736},
  year={2023}
}

@article{wang2024sqdmapnet,
  title={Stream query denoising for vectorized hd map construction},
  author={Wang, Shuo and Jia, Fan and Liu, Yingfei and Zhao, Yucheng and Chen, Zehui and Wang, Tiancai and Zhang, Chi and Zhang, Xiangyu and Zhao, Feng},
  journal={arXiv preprint arXiv:2401.09112},
  year={2024}
}

@InProceedings{Li_2022_DN-DETR,
    author    = {Li, Feng and Zhang, Hao and Liu, Shilong and Guo, Jian and Ni, Lionel M. and Zhang, Lei},
    title     = {DN-DETR: Accelerate DETR Training by Introducing Query DeNoising},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {13619-13627}
}

@inproceedings{zhang2014loam,
  title={LOAM: Lidar odometry and mapping in real-time.},
  author={Zhang, Ji and Singh, Sanjiv and others},
  booktitle={Robotics: Science and systems},
  volume={2},
  number={9},
  pages={1--9},
  year={2014},
}

@inproceedings{shan2018lego,
  title={Lego-loam: Lightweight and ground-optimized lidar odometry and mapping on variable terrain},
  author={Shan, Tixiao and Englot, Brendan},
  booktitle={2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4758--4765},
  year={2018},
  organization={IEEE}
}

@inproceedings{li2022hdmapnet,
  title={Hdmapnet: An online hd map construction and evaluation framework},
  author={Li, Qi and Wang, Yue and Wang, Yilun and Zhao, Hang},
  booktitle={2022 International Conference on Robotics and Automation (ICRA)},
  pages={4628--4634},
  year={2022},
  organization={IEEE}
}

@inproceedings{li2022bevformer,
  title={Bevformer: Learning bird’s-eye-view representation from multi-camera images via spatiotemporal transformers},
  author={Li, Zhiqi and Wang, Wenhai and Li, Hongyang and Xie, Enze and Sima, Chonghao and Lu, Tong and Qiao, Yu and Dai, Jifeng},
  booktitle={European Conference on Computer Vision},
  pages={1--18},
  year={2022},
  organization={Springer}
}

@inproceedings{philion2020lss,
  title={Lift, Splat, Shoot: Encoding Images from Arbitrary Camera Rigs by Implicitly Unprojecting to 3D},
  author={Philion, Jonah and Fidler, Sanja},
  booktitle={European Conference on Computer Vision},
  pages={194--210},
  year={2020},
  organization={Springer}
}

@inproceedings{zhou2022cross,
  title={Cross-view transformers for real-time map-view semantic segmentation},
  author={Zhou, Brady and Kr{\"a}henb{\"u}hl, Philipp},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={13760--13769},
  year={2022}
}

@inproceedings{wang2023bevlanedet,
  title={Bev-lanedet: An efficient 3d lane detection based on virtual camera via key-points},
  author={Wang, Ruihao and Qin, Jian and Li, Kaiying and Li, Yaochen and Cao, Dong and Xu, Jintao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1002--1011},
  year={2023}
}

@inproceedings{chen2022persformer,
  title={Persformer: 3d lane detection via perspective transformer and the openlane benchmark},
  author={Chen, Li and Sima, Chonghao and Li, Yang and Zheng, Zehan and Xu, Jiajie and Geng, Xiangwei and Li, Hongyang and He, Conghui and Shi, Jianping and Qiao, Yu and others},
  booktitle={European Conference on Computer Vision},
  pages={550--567},
  year={2022},
  organization={Springer}
}

@inproceedings{feng2022rethinking_lane_detection,
  title={Rethinking efficient lane detection via curve modeling},
  author={Feng, Zhengyang and Guo, Shaohua and Tan, Xin and Xu, Ke and Wang, Min and Ma, Lizhuang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={17062--17070},
  year={2022}
}

@InProceedings{Qiao_2023_bemapnet,
    author    = {Qiao, Limeng and Ding, Wenjie and Qiu, Xi and Zhang, Chi},
    title     = {End-to-End Vectorized HD-Map Construction With Piecewise Bezier Curve},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2023},
    pages     = {13218-13228}
}

@InProceedings{Ding_2023_pivotnet,
    author    = {Ding, Wenjie and Qiao, Limeng and Qiu, Xi and Zhang, Chi},
    title     = {PivotNet: Vectorized Pivot Learning for End-to-end HD Map Construction},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {3672-3682}
}

@InProceedings{Liu_2024_mgmap,
    author    = {Liu, Xiaolu and Wang, Song and Li, Wentong and Yang, Ruizi and Chen, Junbo and Zhu, Jianke},
    title     = {MGMap: Mask-Guided Learning for Online Vectorized HD Map Construction},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2024},
    pages     = {14812-14821}
}

@article{liu2024mapqr,
  title={Leveraging Enhanced Queries of Point Sets for Vectorized Map Construction},
  author={Liu, Zihao and Zhang, Xiaoyu and Liu, Guangwei and Zhao, Ji and Xu, Ningyi},
  journal={arXiv preprint arXiv:2402.17430},
  year={2024}
}

@article{chen2024polydiffuse,
  title={Polydiffuse: Polygonal shape reconstruction via guided set diffusion models},
  author={Chen, Jiacheng and Deng, Ruizhi and Furukawa, Yasutaka},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{xu2023insightmapper,
  title={Insightmapper: A closer look at inner-instance information for vectorized high-definition mapping},
  author={Xu, Zhenhua and Wong, Kenneth KY and Zhao, Hengshuang},
  journal={arXiv preprint arXiv:2308.08543},
  year={2023}
}

@inproceedings{carion2020detr,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European conference on computer vision},
  pages={213--229},
  year={2020},
  organization={Springer}
}

@article{han2024videobev,
  title={Exploring recurrent long-term temporal fusion for multi-view 3d perception},
  author={Han, Chunrui and Yang, Jinrong and Sun, Jianjian and Ge, Zheng and Dong, Runpei and Zhou, Hongyu and Mao, Weixin and Peng, Yuang and Zhang, Xiangyu},
  journal={IEEE Robotics and Automation Letters},
  year={2024},
  publisher={IEEE}
}

@InProceedings{Wang_2023_streampetr,
    author    = {Wang, Shihao and Liu, Yingfei and Wang, Tiancai and Li, Ying and Zhang, Xiangyu},
    title     = {Exploring Object-Centric Temporal Modeling for Efficient Multi-View 3D Object Detection},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {3621-3631}
}

@InProceedings{He_2016_resnet,
author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
title = {Deep Residual Learning for Image Recognition},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@inproceedings{caesar2020nuscenes,
  title={nuscenes: A multimodal dataset for autonomous driving},
  author={Caesar, Holger and Bankiti, Varun and Lang, Alex H and Vora, Sourabh and Liong, Venice Erin and Xu, Qiang and Krishnan, Anush and Pan, Yu and Baldan, Giancarlo and Beijbom, Oscar},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={11621--11631},
  year={2020}
}

@article{wilson2023argoverse,
  title={Argoverse 2: Next generation datasets for self-driving perception and forecasting},
  author={Wilson, Benjamin and Qi, William and Agarwal, Tanmay and Lambert, John and Singh, Jagjeet and Khandelwal, Siddhesh and Pan, Bowen and Kumar, Ratnesh and Hartnett, Andrew and Pontes, Jhony Kaesemodel and others},
  journal={arXiv preprint arXiv:2301.00493},
  year={2023}
}

@InProceedings{Roddick_2020_nusc_new_split,
author = {Roddick, Thomas and Cipolla, Roberto},
title = {Predicting Semantic Map Representations From Images Using Pyramid Occupancy Networks},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@article{loshchilov2017adamw,
  title={Fixing weight decay regularization in adam},
  author={Loshchilov, Ilya and Hutter, Frank and others}
}

@inproceedings{park2022solofusion,
  title={Time will tell: New outlooks and a baseline for temporal multi-view 3d object detection},
  author={Park, Jinhyung and Xu, Chenfeng and Yang, Shijia and Keutzer, Kurt and Kitani, Kris M and Tomizuka, Masayoshi and Zhan, Wei},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2022}
}

@InProceedings{Zhou_2024_rmem,
    author    = {Zhou, Junbao and Pang, Ziqi and Wang, Yu-Xiong},
    title     = {RMem: Restricted Memory Banks Improve Video Object Segmentation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2024},
    pages     = {18602-18611}
}

@inproceedings{cheng2022xmem,
  title={Xmem: Long-term video object segmentation with an atkinson-shiffrin memory model},
  author={Cheng, Ho Kei and Schwing, Alexander G},
  booktitle={European Conference on Computer Vision},
  pages={640--658},
  year={2022},
  organization={Springer}
}

@article{chen2017dilation,
  title={Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs},
  author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={4},
  pages={834--848},
  year={2017},
  publisher={IEEE}
}

@article{wilson2022motionsc,
  title={MotionSC: Data set and network for real-time semantic mapping in dynamic environments},
  author={Wilson, Joey and Song, Jingyu and Fu, Yuewei and Zhang, Arthur and Capodieci, Andrew and Jayakumar, Paramsothy and Barton, Kira and Ghaffari, Maani},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={3},
  pages={8439--8446},
  year={2022},
  publisher={IEEE}
}

@article{chung2014GRU,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}

@inproceedings{liu2023bevfusion,
  title={Bevfusion: Multi-task multi-sensor fusion with unified bird's-eye view representation},
  author={Liu, Zhijian and Tang, Haotian and Amini, Alexander and Yang, Xinyu and Mao, Huizi and Rus, Daniela L and Han, Song},
  booktitle={2023 IEEE international conference on robotics and automation (ICRA)},
  pages={2774--2781},
  year={2023},
  organization={IEEE}
}

@inproceedings{xie2022working,
  title={Working Memory Capacity Predicts More Effective Problem Space Exploration},
  author={Xie, Xinyu and Moss, Jarrod},
  booktitle={Proceedings of the Annual Meeting of the Cognitive Science Society},
  volume={44},
  number={44},
  year={2022}
}

@inproceedings{zhao2024crkd,
  title={CRKD: Enhanced Camera-Radar Object Detection with Cross-modality Knowledge Distillation},
  author={Zhao, Lingjun and Song, Jingyu and Skinner, Katherine A},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15470--15480},
  year={2024}
}

@article{doherty2019dual,
  title={Dual-task costs in working memory: An adversarial collaboration.},
  author={Doherty, Jason M and Belletier, Clement and Rhodes, Stephen and Jaroslawska, Agnieszka and Barrouillet, Pierre and Camos, Valerie and Cowan, Nelson and Naveh-Benjamin, Moshe and Logie, Robert H},
  journal={Journal of experimental psychology: learning, memory, and cognition},
  volume={45},
  number={9},
  pages={1529},
  year={2019},
  publisher={American Psychological Association}
}

@article{cowan2010magical,
  title={The magical mystery four: How is working memory capacity limited, and why?},
  author={Cowan, Nelson},
  journal={Current directions in psychological science},
  volume={19},
  number={1},
  pages={51--57},
  year={2010},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}


@inproceedings{song2024lirafusion,
  author    = {Song, Jingyu and Zhao, Lingjun and Skinner, Katherine A},
  title     = {LiRaFusion: Deep Adaptive LiDAR-Radar Fusion for 3D Object Detection},
  booktitle={2024 IEEE International Conference on Robotics and Automation (ICRA)},
  year      = {2024},
  pages={18250-18257},
}

